A Tight Estimate for Decoding Error-Probability of LT Codes Using Kovalenko's Rank Distribution

A new approach for estimating the Decoding Error-Probability (DEP) of LT codes with dense rows is derived by using the conditional Kovalenko's rank distribution. The estimate by the proposed approach is very close to the DEP approximated by Gaussian Elimination, and is significantly less complex. As a key application, we utilize the estimates for obtaining optimal LT codes with dense rows, whose DEP is very close to the Kovalenko's Full-Rank Limit within a desired error-bound. Experimental evidences which show the viability of the estimates are also provided.

==> degdesign.tex <==

\section{KFRL and KFRO}\label{kfrlo}

In this section, KFRL and KFRO are derived from the rank-distribution of binary random matrices in   \cite{kv1,kv2,cc,rg}  as probabilistic lower bounds for DEP and MSO, respectively. 

Let $\hat{H}$ be an  $(n+k)\times n $ random matrix over $\mathbb{F}_q$ with the density constraint
\begin{equation}
 \frac{\ln(n)+x}{n}\le \Pr(\hat{h}_{ij}\neq 0) \le 1-\frac{\ln(n)+x}{n}, \label{eq:lnnx}
\end{equation}
where $x\to \infty$ arbitrarily slowly. For notation convenience, let  $\xi_k(n-s)=\Pr(\text{Rank}(\hat{H})=n-s|k+s\ge 0)$.
 It was shown   in \cite{kv1} by Kovalenko that 
\begin{equation}
\lim_{n\to\infty} \xi_k (n-s) = \frac{1}{q^{s(k+s)}}
 \frac{ \prod_{i=s+1}^{\infty} (1-\frac{1}{q^i})}
      {\prod_{i=1}^{k+s} (1-\frac{1}{q^i})}.       \label{eq:qrd}
\end{equation} 
It  was shown further in \cite{cc} by Cooper that, under the assumption that $\hat{H}$ has no zero columns, the limit distribution (\ref{eq:qrd}) still holds when $x\to -\infty$ arbitrarily slowly.  


Let $\hat{H}$ be now an  $m\times n$ binary random matrix  that consists of random rows $\hat{H}_i=(\hat{h}_{i1},\dots,\hat{h}_{in})$, $i=1,\dots,m$, such that $\Pr(\hat{h}_{ij}=1)=\frac{1}{2}$, $j=1,\dots,n$. With $q=2$, we have 
\begin{equation}
 \xi_k(n-s)=\frac{S(n-s,k+s)}{2^{s(k+s)}} \prod_{i=s+1}^{n}\left(1-\frac{1}{2^i} \right), \label{eq:krt}
\end{equation} 
where, with $l=k+s$,
\begin{equation}
  S(n-s,l)=  \sum_{i_{1}=0}^{n-s}2^{-i_{1}}\sum_{ i_{2}=i_{1}}^{n-s}2^{-i_{2}}\cdots \sum_{i_l=i_{l-1}}^{n-s}2^{-i_l}. \label{eq:mkvsumr}
\end{equation} 
Since the sequence $\{S(n-s,k+s) \}_{n=s}^{\infty}$ is increasing and $\lim_{n\to\infty}S(n-s,k+s)=\prod_{i=1}^{k+s}(1-\frac{1}{2^i})^{-1}$, we have
\begin{equation}
\xi_{k}(n-s) \le \frac{1}{2^{s(k+s)}} \frac{\prod_{i=s+1}^{n}\left(1-\frac{1}{2^i} \right)}{\prod_{i=1}^{k+s}\left(1-\frac{1}{2^i} \right)}. \label{eq:n-s}
\end{equation}
%where the right-hand side is a finite case of (\ref{eq:qrd}) with $q=2$.  
The KFRL defined in (\ref{eq:kfrl0}) comes from the upper-bound above with $s=0$ holding the inequality
\begin{equation}
K(1+\gamma,n) \le \left( 1-\xi_{k}(n)=\Pr(\text{Rank}(\hat{H})<n)\right), \label{eq:kfrl}
\end{equation}
where $\gamma=\frac{k}{n}$.  The KFRO  defined in (\ref{eq:kfro0}) is then the minimum $\gamma$ satisfying the constraint $ K(1+\gamma,n)\le \delta$.
% Notice that KFRL is decreasing with respect to $\gamma$, and thus,  $K(1+\gamma,n)\le \delta$ for any $\gamma \ge \gamma_K(\delta,n)$.
%Observe that  KFRL  in (\ref{eq:kfrl}) can be computed explicitly, and consequently, $\gamma_K(\delta,n)$ is obtainable from the graph of $K(1+\gamma,n)$ for any $\delta>0$. 

For a given $\delta >0$, let $k_\delta$ be the smallest integer such that $2^{-k}\le \delta$.  Then with $m=n+k_\delta$ for the row-dimension of $\hat{H}$, it holds that $\Pr(\text{Rank}(\hat{H})<n)\le \frac{1}{2^{k_\delta}} \le \delta$ (see \cite[Ex.50.11]{mackay2}). Hence  by the inequality in (\ref{eq:kfrl}) and by the definition of KFRO in (\ref{eq:kfro0}), 
\begin{equation}
\gamma_K(\delta,n)\le \frac{k_\delta}{n}  \le  \frac{1+\log_2(1/\delta)}{n}.
\end{equation} 
Interestingly, although the authors of the paper have no mathematical proofs yet,  experiments exhibited that  $K(1+\gamma,n)$ is almost identical to  $2^{-\gamma n}$ as $\gamma$ increases. (See their graphs in  \figref{fig:DefNPerf2} for $n=100$). 
Therefore  $\gamma_K(\delta,n):=\frac{k_\delta}{n}$ for small $\delta$. 


 The following theorem shows KFRL and KFRO as lower-bounds for DEP in (\ref{eq:dfr0}) and MSO in (\ref{eq:mo}), respectively. For the proof, see {\bf Lemma~2.1} and {\bf Theorem~2.2} in \cite{kfrl}.
 
\begin{thm1}\label{thm:frb} Let $\rho(x)$ be of the form in (\ref{eq:rho1}). 
Then $K(1+\gamma, n) \le \dpr(1+\gamma,n,\rho)$, and thus, $\gamma_{\min}(\delta,n,\rho) \ge   \gamma_K(\delta,n)$.  
%\begin{equation}
% K(1+\gamma, n) \le \dpr(1+\gamma,n,\rho), \label{ineq:kfrl}
%\end{equation}
%and therefore,
%\begin{equation}
%\gamma_{\min}(\delta,n,\rho) \ge   \gamma_K(\delta,n). \label{eq:mfo}
%\end{equation}
For successful decoding  with a destined constraint $\dpr(1+\gamma,n,\rho)\le \delta$, therefore, the number of syndrome symbols  that a receiver should acquire is at least $(1+\gamma_K(\delta, n))n$.
\end{thm1}



 \label{eg:2}\begin{eg1} Let $\delta=10^{-4}$.
From  $K(1+\gamma,100)$ in  \figref{fig:DefNPerf2}, we have $\gamma_K(10^{-4},100):=0.14$ (and also $k_\delta:=14$).
Thus $\gamma_{\min}(10^{-4},100,\rho) \ge 0.14$ by {\bf Theorem~\ref{thm:frb}}.  
To meet a destined constraint  $\dpr(1+\gamma,100,\rho)\le 10^{-4}$, therefore, the number of symbols of $\beta$ of  \sysref{sys:ltini} that a receiver should acquire is at least $100\cdot (1.14)=114$. 
\hfill \IEEEQEDclosed
\end{eg1}





\section{Degree-Distribution Design with Dense Rows} \label{degdesign}

In this section, an RSD $\mu(x)$ is explained by Mackay's recursion in \cite[Ex.50.2]{mackay2} first; a truncation of $\mu(x)$ is considered for an optimal $\rho(x)$ in (\ref{eq:rho1}) second; and then, an optimal  $\rho(x)$ is accomplished with an appropriate $\rho_{n/2}$ by looking at KFRL, KFRO, and UBDEP for various fractions for $\rho_{n/2}$.


Let $H$ of \sysref{sys:ltini} be  generated by an RSD $\mu(x)$.  
The recursion  can be derived by tracing out row-degrees of residual matrices induced by the diagonal extension process stated in \algoref{algo:alta}.  
At round $t$ of the diagonal extension process, starting from $H[0]:=H$, let $H[t]$ denote the residual matrix of $H[t-1]$ by discarding the ${j_t}^{th}$ column and the ${i_t}^{th}$ row of $H[t-1]$ as $1_{i_t,j_t}$ is selected for the $t^{th}$ diagonal entry of $B$ in \sysref{sys:bsr0}. 
Let $h_t(d)$ denote the expected number of rows of  degree $d$ in $H[t]$. 
Then with  $h_t(1) \ge 1$ for all $t$, we have the recursion
\begin{equation}
h_{t+1}(d)=
 \begin{cases}
   (h_t(1)-1)\left(1-\frac{1}{n-t}\right) + \frac{2h_t(2)}{n-t}, & \text{if} \; d=1\\
    h_t(d)\left(1-\frac{d}{n-t}\right) + \frac{(d+1)h_t(d+1)}{n-t}, & \text{otherwise} 
 \label{eq:htd}
 \end{cases}.
\end{equation}
Setting $h_t(1)=S+1$ above for all $t$ yields the solution
\begin{equation}
h_t(d)=\frac{n-t}{d(d-1)}+ \frac{S}{d}, \quad d>1. \label{htd}
\end{equation}
When $t=0$, in particular,  the expected number of rows of degree $d$ in $H$ is given as
\begin{equation}
 h_0(d)=
  \begin{cases}
    S+1, & \text{if } d=1 \\
    \frac{n}{d(d-1)} + \frac{S}{d}, &\text{otherwise} \label{h0d}
  \end{cases}.
\end{equation}
Setting  the number of rows of $H$ as
\begin{equation}
m=\sum_{d=1}^n h_0(d) \approx n+ S(1+\ln(n)), \label{eq:numr}
\end{equation}
then normalizing $h_0(d)$ by the $m$ yields an RSD as
\begin{equation}
 \mu(x)=\sum_{d=1}^n \mu_d x^d, \quad \text{where} \quad \mu_d=\frac{h_0(d)}{m}. \label{eq:grsd} 
\end{equation}

The Ideal Soliton Distribution in \cite{lt} is a particular case of $\mu(x)$ above with $S=0$, and 
the RSD in \cite{lt} can be understood as a truncation with  $S=c\ln(n/\delta)\sqrt{n}$  in such a way that
\begin{equation}
h_0(d)=\begin{cases} 
                  \frac{n}{d(d-1)} + \frac{S}{d}, & 1 < d < \frac{n}{S},\\
                  \frac{n}{d(d-1)} + \underbrace{S\ln(S/\delta)}_{\text{a spike}}, & d= \frac{n}{S},\\   
                  \frac{n}{d(d-1)} & \text{otherwise}. 
       \end{cases} \label{eq:ch0}
\end{equation}
 {\bf Theorem-17} in \cite{lt} guarantees that,  when $H$ is generated by  the normalization of (\ref{eq:ch0}) with $m \approx n+S\ln(n/\delta)$,  \sysref{sys:ltini}  can be solved for $X=\alpha$ by the MPA alone with the success probability that is at least $1-\delta$.  


In practice,  most of the fractions  of $\mu(x)$ in (\ref{eq:grsd}) are too small to get $ m\mu_d \ge 1$. 
Hence  fractions for higher degrees like the spike term in (\ref{eq:ch0}) should be assigned appropriately to meet a certain constraint on $|H|$, so that a random $H$ by $\mu(x)$ gets no zero columns with high probability.
Let $\mu(x)$ be now a truncated RSD such that $\mu(x)=\sum_{d\le d_0}\mu_d x^d$ where $\lim_{n\to\infty}\frac{d_0}{n}=0$.
A density constraint of a random $H$ generated by $\mu(x)$ can be derived by looking at the column-degree distribution of $H$. 
The column-degree distribution, say $\lambda(x)$,  can be derived by the following arguments.
First, when a row $H_i$ of degree $d_i$ is generated,  a column of $H$ increases its degree by one with probability $\frac{d_i}{n}$. Let $f_{d_i}(x)=(d_i/n)x+(1-d_i/n)$. Since every row of $H$ is generated in random independently from all other rows, we have $\lambda(x)=\prod_{i=1}^{m} f_{d_i}(x)$.
Second, $H$ follows the row-degree distribution $\mu(x)$,  rearranging the product with respect to degree $d$ yields 
\begin{equation}
  \lambda(x)=\prod_{d=1}^{d_0} \left[\left(1-\frac{d}{n}\right)+\left(\frac{d}{n}\right)x\right]^{(1+\gamma)n \mu_d}. \label{eq:lambda}
\end{equation} 
The expected number of null columns of $H$, that is $n\lambda(0)$, can then be approximated as $ne^{-(1+\gamma)\sum d\mu_d}$.  
With an appropriate $d_0$, thus, fractions of $\mu(x)$ can be assigned to meet the constraint $n\lambda(0) \le \delta<1$ for some $\delta$, that is equivalent to 
\begin{equation}
a_r=\sum_{d\le d_0} d\cdot \mu_d  \quad \ge \quad \frac{\ln(n/\delta )}{(1+\gamma)}, \label{eq:avg}
\end{equation}
where $a_r$ is the average row-degree of $H$. 
By doing so, $H$ gets no zero columns with probability at least $1-\delta$.


For short $n$, however, experiments exhibited that the DEP of LT codes by a truncated $\mu(x)$ alone floors over a large range of $\gamma$, even if $\mu(x)$ meets the constraint (\ref{eq:avg}).
For example, the curve $\dpr(1+\gamma,100,\mu)$ in \figref{fig:DefNPerf1} is an estimated DEP of LT codes generated by the $\mu(x)$ in \tabref{tab:rho}, and it never reaches $10^{-3}$ for $1+\gamma \le 1.3$.  
 A desirable feature of $\mu(x)$ is however that, for $\gamma \ge 0$, the DEP  is mainly contributed by the rank-deficient probabilities  $\Pr(\text{Rank}(H)=n-\eta)$ of  small $\eta$.
 For example, see the curves  $\eta=1,\dots,6$ in \figref{fig:DefNPerf1}.  
These deficient probabilities become very small when enough number of dense rows are supplemented to $H$. 
The portion of the density $|H|$ contributed by  supplemented dense rows alone however could be much larger than expected.  
Therefore, the number of dense rows should be  small as possible, while maintaining the MSO  $\gamma_{\min}(\delta,n,\rho)$ near  the KFRO $\gamma_K(\delta,n)$.  




 
\begin{table}[t]
\begin{center}
\centering
\begin{tabular}{|c|l|}
 \hline%\hline
$\mathcal{D}_1$  & $(\mu_d)_{d=1}^{10}=(0.014,0.481,0.152,0.082,0.048,0.034,0.024,0.024,0.012,0.012)$ \\   
%$\mathcal{D}_1$  & $(\mu_d)_{d=6}^{10}=(0.034,0.024,0.024,0.012,0.012)$\\ 
 \hline
$\mathcal{D}_2$  & $\mu_{25}=0.059$, $\mu_{35}=0.058$ \\ 
 \hline
\end{tabular}
\end{center}
\caption{Fractions of $\mu(x)$  generated by the steps R1) and R2) with $S=10$ and $n=10^3$. \label{tab:rho}}
\end{table} 

%\begin{table}[t]
%\begin{center}
%\begin{tabular}{|c|l|}
% \hline%\hline
%                 & $(\mu_d)_{d=1}^{5}=(0.014,0.481,0.152,0.082,0.048)$ \\   
%$\mathcal{D}_1$  & $(\mu_d)_{d=6}^{10}=(0.034,0.024,0.024,0.012,0.012)$\\ 
% \hline
%$\mathcal{D}_2$  & $\mu_{25}=0.059$, $\mu_{35}=0.058$ \\ 
% \hline
%\end{tabular}
%\end{center}
%\caption{Fractions of $\mu(x)$  generated by the steps R1) and R2) with $S=10$ and $n=10^3$. \label{tab:rho}}
%\end{table}

Let us clarify several notations that shall be conveniently used in \thmref{thm:upmu}. 
 Let  $H$ be now an $m\times n$ random matrix generated by $\rho(x)$  in (\ref{eq:rho1}).
By rearranging rows, $H$ can be expressed as $H=\left[\begin{smallmatrix} \tilde{H} \\ \hat{H} \end{smallmatrix} \right]$, where  $\tilde{H}$ is a sparse  matrix generated by a truncated $\mu(x)$ and  $\hat{H}$ is  a dense  matrix generated by the row-degree distribution $x^{n/2}$.
Let $B(m,k,p)=\binom{m}{k}p^k (1-p)^{m-k}$ the Bernouli probability with $0\le p<1$.   Assume that $\hat{H}$  attains $k$ rows with probability $B(m,k,\rho_{n/2})$.
With the sparse part $\tilde{H}$, let $\varphi_{\mu}(\eta)=\Pr(\text{Rank}(\tilde{H})=n-\eta)$. 
Let $\vartheta_{\rho} (k,\eta)=\Pr(\text{Rank}(H)<n|k,\eta)$  the conditional probability that $\text{Rank}(H)<n$, given that $\hat{H}$ attains $k$ rows and $\text{Rank}(\tilde{H})=n-\eta$. 
Finally, let $\vartheta_{\rho} (k)=\Pr(\text{Rank}(H)<n|k)$ the conditional probability that $\text{Rank}(H)<n$ given that $\hat{H}$ has $k$ rows.
Then we have
  \begin{equation}
  \dpr(1+\gamma,n,\rho) = \sum_{k=0}^{m}B(m,k,\rho_{n/2})\cdot \vartheta_{\rho} (k),
 \end{equation}
 where
\begin{equation} 
 \vartheta_\rho(k)=\sum_{\eta=1}^{n} \vartheta_\rho(k,\eta)\cdot \varphi_{\mu}(\eta).
\end{equation} 
\begin{thm1}[The UBDEP of LT codes generated by $\rho(x)$]\label{thm:upmu} Using the notations and conditions so far, we have $\vartheta_{\rho} (k,\eta)\le \frac{1}{2^{k-\eta}}$ for $1\le\eta\le k$ and $\vartheta_{\rho} (k,\eta)=1$ for $\eta>k$, and therefore,
\begin{equation}
\vartheta_{\rho} (k) \le \left( \overline{\vartheta_{\rho} (k)}=\sum_{\eta=1}^{k} \frac{\varphi_\mu(\eta)}{2^{k-\eta}} + \sum_{\eta >k}\varphi_\mu(\eta)\right). \label{eq:cdrdef}
\end{equation}
This leads us that
\begin{equation}
 \dpr(1+\gamma,n,\rho) \le \sum_{k=0}^{m}B(m,k,\rho_{n/2})\cdot \overline{\vartheta_{\rho} (k)}. \label{eq:udep}
\end{equation}
\end{thm1}

\begin{IEEEproof}
Showing $\vartheta_\rho(k,\eta) \le \frac{1}{2^{k-\eta}}$ is enough for the proof. 
Note that  $\text{Rank}(H)< n$ iff. 
 $\hat{H}\cdot V^T=0$ for some $V\neq 0$ in $\text{Ker}(\tilde{H})$, where $\tilde{H}$ and $\hat{H}$ are the sparse and the dense part of $H$, respectively. 
For a nonzero $V$ in $\text{Ker}(\tilde{H})$, since each row of $\hat{H}$ is generated independently from all other rows of $H$ and $V$ with degree $\frac{n}{2}$, $\Pr(\hat{H}\cdot V^T=0)=2^{-k}$.  
Then the union bound  with $|\text{Ker}(\tilde{H})|= 2^{\eta}$ asserts that $\vartheta_\rho(k,\eta) \le \frac{1}{2^{k-\eta}}$.
\end{IEEEproof}


 The UBDEP  in (\ref{eq:udep}) is very practical  in that, once the deficient probabilities $\Pr(\text{Rank}(\tilde{H})=n-\eta)$ are estimated over a deficiency-range $0< \eta <\eta_0$, the UBDEP  can be estimated  explicitly  within a second for any $\rho_{n/2}$.  Furthermore, the estimate is close to the DEP $\dpr(1+\gamma,n,\rho)$. 
Thus, the overall shape of the DEP is predictable  by the estimate  without exhaustive experiments for DEP.  Consequently,  for any error-performance bound $\delta$, an optimal $\rho(x)$ can be found as desired by checking the estimates with various values of $\rho_{n/2}$.  

The following example shows how to optimize $\rho(x)$ with the $\mu(x)$ in \tabref{tab:rho} using UBDEP's in \thmref{thm:upmu}. 
\begin{eg1}
In \figref{fig:DefNPerf1}, the deficiency curves  $\eta=1,2,3,\dots,$  represent  $\Pr(\text{Rank}(\tilde{H})=n-\eta)$ for $n=100$ that are estimated by the S-MLDA over \sysref{sys:ltini}. 
In \figref{fig:DefNPerf2}, dashed curves  are estimated UBDEP's in (\ref{eq:udep}) for $\rho_{n/2}=0.05,0.10,0.15$ by using the finite UBDEP
\begin{equation}
\sum_{k=l-5}^{l+5}B(m,k,\rho_{\frac{n}{2}})\left( \sum_{\eta=1}^{k} \frac{\varphi_\mu(\eta)}{2^{k-\eta}} + \sum_{\eta =k+1}^{30} \varphi_\mu(\eta)\right),
\end{equation}
where $l=\left\lfloor m\rho_{\frac{n}{2}}\right\rfloor$.
 The blue  curves in the figure represent $\dpr(1+\gamma,100,\rho)$ obtained by exhaustive experiments under the S-MLDA over \sysref{sys:ltini}, in which $H$ is generated by $\rho(x)$ with $\rho_{n/2}=0.05,0.10, 0.15$. 

Let $\delta=10^{-4}$. 
By \thmref{thm:upmu}, the smallest MSO  with this error-bound should be larger than the KFRO $\gamma_K(10^{-4},100)=0.14$ (see \figref{fig:DefNPerf2}).  
Assume we want a $\rho(x)$ such that   $0.14\le\gamma_{\min}(10^{-4},100,\rho)\le 0.16$. 
As shown in \figref{fig:DefNPerf2}, an UBDEP for $\rho_{n/2}\le 0.10$ does not reach the bound $\delta=10^{-4}$ for $1+\gamma\le 1.16$.  Therefore,  $\rho_{n/2}\ge 0.10$ in this case. 
The UBDEP  for  $\rho_{n/2}=0.15$ yields that, without experiments for DEP, $\gamma_{\min}(1+\gamma,100,\rho)\le 0.16$ for any $\rho_{n/2}\ge 0.15$. 
With $\delta=10^{-6}$ and $\gamma_{\min}(10^{-6},100,\rho)\le 0.22$, similarly, it can be found right away from the UBDEP for $\rho_{n/2}=0.20$ that $\rho_{n/2}= 0.20$ is large enough for an optimal $\rho(x)$. \hfill \IEEEQEDclosed
\end{eg1}


%One last thing should be observed from the figure is that, larger dense fractions  $\rho_{n/2}$ exhibits closer DEP $\dpr(1+\gamma,100,\rho)$  to the ideal limit $K(1+\gamma,100)$.

It should be emphasized in \figref{fig:DefNPerf1} that the curve $\dpr(1+\gamma,100,\mu)$  emerges to the  curve $\eta=1$ as $\gamma$ increases. 
Therefore, only one or two rows of $\hat{H}$ are actually used for the full-rank of $H$ and the rest of them become redundant after the pre-decoding stage. 
 Therefore, the number of symbol-additions made during the post-decoding  is mainly contributed by  the sparse density $|\tilde{H}|$, because symbol-additions over redundant rows including most of dense rows of $\hat{H}$ are removed at the  post-decoding, albeit inevitable at encoding process.


\begin{figure}
 \centering
 \subfigure[]{ \fbox{\epsfig{file=RD100_mu.eps, width=7.8cm,height=5.7cm}} \label{fig:DefNPerf1}}
 \subfigure[]{\fbox{\epsfig{file=UDEPrho100.eps, width=7.8cm,height=5.7cm}}\label{fig:DefNPerf2}}
\caption{ In (a), each curve represents an estimated $\Pr(\text{Rank}(H)=n-\eta)$ under the S-MLDA, where $H$ generated by the $\mu(x)$ in \tabref{tab:rho}.  The plots are based on $10^7$ random constructions of \sysref{sys:ltini} for each $1+\gamma$.  In (b), curves represent KFRL (red), UBDEP (dashed), and DEP of LT codes by $\rho(x)$ (blue) with $n=100$. In the figure, $\rho(x)$ is a supplementation of the $\mu(x)$ in \tabref{tab:rho} with   various fractions for $\rho_{50}$.
} 

\end{figure}


%\begin{figure}[t]
% \centerline{ \fbox{\epsfig{file=RD100_mu.eps, width=8.5cm,height=6cm}}}
%\caption{  \label{fig:DefNPerf1}  
%Each curve represents an estimated $\Pr(\text{Rank}(H)=n-\eta)$ under the S-MLDA, where $H$ generated by the $\mu(x)$ in \tabref{tab:rho}.  The plots are based on $10^7$ random constructions of \sysref{sys:ltini} for each $1+\gamma$. 
%}
%\end{figure}  
% 
%\begin{figure}[t] 
%
% \centerline{ \fbox{\epsfig{file=UDEPrho100.eps, width=8.5cm,height=6cm}}}
%\caption{ \label{fig:DefNPerf2} Curves represent KFRL (red), UBDEP (dashed), and DEP of LT codes by $\rho(x)$ (blue) with $n=100$. In the figure, $\rho(x)$ is a supplementation of the $\mu(x)$ in \tabref{tab:rho} with   various fractions for $\rho_{50}$.
%} 
%\end{figure}



Let $\mcd_1=\{1,2,\dots, d_s \}$, and  let $\mcd_2$ be a set of few spike  degrees $d$ such that $d_s < d \le d_0$ for some $d_0$. 
An optimal construction of $\rho(x)$  in (\ref{eq:rho1}) is summarized as follows.  
\begin{enumerate}[\; R1)]
 \item Generate $\mu(x)$  in (\ref{eq:grsd}) with  desired $S$ and $n$. 
 \item  Take  a few spike terms for $\mcd_2$ in such a way that $\sum_{d\in\mcd_2}\mu_d = 1- \sum_{d\in \mcd_1}\mu_d$;
 \item Choose a smaller  $\rho_{n/2}=\frac{\kappa}{1+\kappa}$  as desired by using the UBDEP of \thmref{thm:upmu}. Then set 
\begin{equation}
 \rho(x)=\sum_{d\in \mathcal{D}_1\cup\mathcal{D}_2} \left(\frac{\mu_d}{1+\kappa} \right) x^d + \left(\frac{\kappa}{1+\kappa} \right)x^{\frac{n}{2}}. \label{eq:arsd}
\end{equation}
\end{enumerate}
 The fractions of degrees in $\mcd_1$ and $\mcd_2$ are aimed for a larger triangular block $B$ of $\bar{H}$  in \sysref{sys:ps1}, and at the same time to hold   $\sum_{d\in\mathcal{D}_1\cup\mcd_2}d\rho_d \ge \frac{\ln(n)}{1+\gamma}$. Thus, hopefully, most of columns of $H$, except one or two of them, have a  one in some rows  of degree $d \in \mcd_1 \cup \mcd_2$.
An exemplary $\mu(x)$  made by the steps R1) and R2) is listed in \tabref{tab:rho}, and its supplementation $\rho(x)$ was used for computer simulations  with various values of $\rho_{n/2}$ (see  \figref{fig:DefNPerf2}).  





